Private Interdependent Valuations

We consider the single-item interdependent value setting, where there is a monopolist, $n$ buyers, and each buyer has a private signal $s_i$ describing a piece of information about the item. Each bidder $i$ also has a valuation function $v_i(s_1,\ldots,s_n)$ mapping the (private) signals of all buyers to a positive real number representing their value for the item. This setting captures scenarios where the item's information is asymmetric or dispersed among agents, such as in competitions for oil drilling rights, or in auctions for art pieces. Due to the increased complexity of this model compared to standard private values, it is generally assumed that each bidder's valuation function $v_i$ is public knowledge. But in many situations, the seller may not know how a bidder aggregates signals into a valuation. In this paper, we design mechanisms that guarantee approximately-optimal social welfare while satisfying ex-post incentive compatibility and individual rationality for the case where the valuation functions are private to the bidders. When the valuations are public, it is possible for optimal social welfare to be attained by a deterministic mechanism under a single-crossing condition. In contrast, when the valuations are the bidders' private information, we show that no finite bound can be achieved by any deterministic mechanism even under single-crossing. Moreover, no randomized mechanism can guarantee better than an $n$-approximation. We thus consider valuation functions that are submodular over signals (SOS), introduced in the context of combinatorial auctions in a recent breakthrough paper by Eden et al. [EC'19]. Our main result is an $O(\log^2 n)$-approximation for buyers with private signals and valuations under the SOS condition. We also give a tight $\Theta(k)$-approximation for the case each agent's valuation depends on at most $k$ other signals even for unknown $k$.

==> impossibility.tex <==
Let $v_i=\beta_{i1}s_1+\beta_{i2}s_2+\beta_{i3}$ and let $s_i\in \{0,1\}$ for $i\in\{1,2\}$. We fist characterize conditions on payments any mechanism ex-post IC mechanism has to fulfill.
\begin{comment}
\begin{lemma}
For $\vec{\beta},\vec{s},$ we have $$p_i(\vec{\beta},\vec{s})-p_i(0_{ij},\vec{\beta}_{-ij},\vec{s})=v_i(\vec{\beta},\vec{s})\cdot x_i(\vec{\beta},\vec{s}) - v_i(0_{ij},\vec{\beta}_{-ij},\vec{s})\cdot x_i(0_{ij},\vec{\beta}_{-ij},\vec{s}) -\int_0^{\beta_jj}x_i(t,\vec{\beta}_{-ij},\vec{s})v_i'(t,\vec{\beta}_{-ij},\vec{s})dt.$$
\end{lemma}  
\end{comment}

\begin{lemma}
	Whenever $\vec{s}=\vec{1}$, any ex-post IC mechanism is monotone in $\beta_{ij}$ for every $i\in \{1,2\}$, $j\in \{1,2\}$. 
\end{lemma}
\begin{proof}
	The proof is by the well known Myerson's Lemma. Consider any $\beta_{ij}'<\beta_{ij}$ with value $v_i'<v_i$. Any truthful mechanism should satisfy
	\begin{align}
		x_i(\beta_{ij}', \vec{\beta}_{-ij}, \vec{s}) v_i' - p_i(\beta_{ij}', \vec{\beta}_{-ij}, \vec{s}) \ge x_i(\beta_{ij}, \vec{\beta}_{-ij}, \vec{s}) v_i' - p_i(\beta_{ij}, \vec{\beta}_{-ij}, \vec{s}), \label{eqn:imp_lem1_eq1}\\
		x_i(\beta_{ij}, \vec{\beta}_{-ij}, \vec{s}) v_i - p_i(\beta_{ij}, \vec{\beta}_{-ij}, \vec{s}) \ge x_i(\beta_{ij}', \vec{\beta}_{-ij}, \vec{s}) v_i - p_i(\beta_{ij}', \vec{\beta}_{-ij}, \vec{s}),  \label{eqn:imp_lem1_eq2}
	\end{align}
	Subtracting the two inequalities we get
	$$
	x_i(\beta_{ij}', \vec{\beta}_{-ij}, \vec{s})(v_i'-v_i)\ge x_i(\beta_{ij}, \vec{\beta}_{-ij}, \vec{s})(v_i'-v_i),
	$$
	which leads to $x_i(\beta_{ij}', \vec{\beta}_{-ij}, \vec{s})\le x_i(\beta_{ij}, \vec{\beta}_{-ij}, \vec{s})$.
\end{proof}

\begin{lemma}
	Fix a deterministic \shuran{and ex-post IC} allocation rule $x$. Let $\vec{s}=1$, and let $x_i(\vec{\beta},\vec{s})=1$.
	Let $\beta_{ij}^*$ be the minimal value of $\beta_{ij}$ for which $x_i(\beta_{ij}^*, \vec{\beta}_{-ij},\vec{s})=1$. Then the payment function of agent $i$ satisfies $$p_i(\beta_{ij}, \vec{\beta}_{-ij}, \vec{s}) = p_i(0_{ij}, \vec{\beta}_{-ij}, \vec{s}) + \beta_{ij}^* + \sum_{\ell\neq j}\beta_{i\ell}.$$
\end{lemma}
\begin{proof}
	Let $\beta_{ij} = \beta_{ij}'+\varepsilon$ in~\eqref{eqn:imp_lem1_eq1} and \eqref{eqn:imp_lem1_eq2} and take the limit $\varepsilon \to 0$ we will get 
	$
	\frac{\text{d} p_i(\beta_{ij}, \vec{\beta}_{-ij}, \vec{s})}{\text{d} \beta_{ij}} = v_i \cdot \frac{\text{d} x_i(\beta_{ij}, \vec{\beta}_{-ij}, \vec{s})}{\text{d} \beta_{ij}}.
	$
	Therefore $p_i(\beta_{ij}, \vec{\beta}_{-ij}, \vec{s}) = p_i(0_{ij}, \vec{\beta}_{-ij}, \vec{s}) + \int_{0}^{\beta_{ij}} v_i(t) x_i'(t,\vec{\beta}_{-ij}, \vec{s})\, \text{d} t$. Since $x_i(t,\vec{\beta}_{-ij}, \vec{s}) = 0$ when $t<\beta_{ij}^*$ and $x_i(t,\vec{\beta}_{-ij}, \vec{s}) = 1$ when $t\ge \beta_{ij}^*$, we have $p_i(\beta_{ij}, \vec{\beta}_{-ij}, \vec{s}) = p_i(0_{ij}, \vec{\beta}_{-ij}, \vec{s}) +  v_i(\beta_{ij}^*)$.
\end{proof}

\begin{corollary}~\label{cor:utility}
	Fix a deterministic \shuran{and ex-post IC} allocation rule $x$. Let $\vec{s}=1$, and let $x_i(\vec{\beta},\vec{s})=1$.
	Let $\beta_{ij}^*$ be the minimal value of $\beta_{ij}$ for which $x_i(\beta_{ij}^*, \vec{\beta}_{-ij},\vec{s})=1$. Then the utility of agent $i$ \shuran{when everyone truthfully reports} is $\beta_{ij}-\beta_{ij}^* - p_i(0_{ij}, \vec{\beta}_{-ij}, \vec{s})$.
\end{corollary}
\begin{proof}
	The value of agent $i$ from winning is $\beta_{ij} + \sum_{\ell\neq j}\beta_{i\ell}$, while the payment of agent $i$ is $p_i(0_{ij}, \vec{\beta}_{-ij}, \vec{s}) +\beta_{ij}^* + \sum_{\ell\neq j}\beta_{i\ell}$.
\end{proof}

\begin{lemma}\label{lem:dependency}
	%Assuming that $p_i(\vec{\beta}, \vec{s}) = 0$ whenever $x_i(\vec{\beta}, \vec{s}) = 0$, 
	There is no deterministic ex-post IC allocation rule $x$ for which for some $\vec{\beta}$ and $\vec{s}=\vec{1}$, where $x_i(\vec{\beta},\vec{s})=1$, $x_i(\beta'_{ii}, \vec{\beta}_{-ii},\vec{s})=0$ for some $\beta'_{ii} < \beta_{ii}$, and  $x_i(\beta'_{ij}, \vec{\beta}_{-ij},\vec{s})=0$ for some $\beta'_{ij} < \beta_{ij}$.
\end{lemma}
\begin{proof}
	Suppose there is such an allocation rule $x$ as described in the lemma statement. Let $\s$, $\beta$ as described by the lemma, and let $\beta^*_{ii}$ and $\beta^*_{ij}$ bet the lowest values for which $x_i(\beta^*_{ii}, \vec{\beta}_{-ii},\vec{s})=1$ and  $x_i(\beta^*_{ij}, \vec{\beta}_{-ij},\vec{s})=1$. According to Corollary~\ref{cor:utility}, the utility of agent $i$ \shuran{when everyone truthfully reports} should satisfy $u_i = \beta_{ii}-\beta^*_{ii} - p_i(0_{ii}, \vec{\beta}_{-ii}, \vec{s})$, and $u_i=\beta_{ij}-\beta^*_{ij} - p_i(0_{ij}, \vec{\beta}_{-ij}, \vec{s})$, which implies 
	\begin{eqnarray}
		\beta_{ii}-\beta^*_{ii} - p_i(0_{ii}, \vec{\beta}_{-ii}, \vec{s})=\beta_{ij}-\beta^*_{ij} - p_i(0_{ij}, \vec{\beta}_{-ij}, \vec{s}).\label{eq:utility_eq1}
	\end{eqnarray}
	
	On the other hand, by monotonicity, we have that for $\hat{\beta}_{ii} > \beta_{ii}$, $x_i(\hat{\beta}_{ii}, \vec{\beta}_{-ii},\vec{s})=1$.  Then by Corollary~\ref{cor:utility} again, \shuran{the utility of agent $i$ with coefficient $\hat{\beta}_{ii}$ should satisfy $\hat{u}_i = \hat{\beta}_{ii}-\beta^*_{ii} - p_i(0_{ii}, \vec{\beta}_{-ii}, \vec{s})$, and $\hat{u}_i=\beta_{ij}-\beta^*_{ij} - p_i(0_{ij}, \hat{\beta}_{ii}, \vec{\beta}_{-ij,ii}, \vec{s})$, the following equation does not hold.}
	\begin{eqnarray*}
		\hat{\beta}_{ii}-\beta^*_{ii} - p_i(0_{ii}, \vec{\beta}_{-ii}, \vec{s})=\beta_{ij}-\beta^*_{ij} - p_i(0_{ij}, \vec{\beta}_{-ij}, \vec{s}),
	\end{eqnarray*}
	contradicting Equation~\eqref{eq:utility_eq1}.
\end{proof}

Assume there exists a deterministic mechanism that achieves better than $c$-approximation.
Consider $v_1 = c s_1 + s_2/c$ and $v_2 = s_2$, and signals $\vec{s}=\vec{1}$. Notice that at that signal profile agent $1$ must be allocated in order to achieve the approximation guarantee. Moreover, notice that since the mechanism achieves a better than $c$ approximation, there exists some $\beta_{11}^*>0$ such that $x_1(\beta_{11}^*, \vec{\beta}_{-11},\vec{s})=1,$ and $x_1(\beta'_{11}, \vec{\beta}_{-11},\vec{s})=0$ for every  $0\leq\beta'_{11}\leq \beta_{11}^*$. By Lemma~\ref{lem:dependency}, $x_1(\beta_{11}^*,0_{12}, \vec{\beta}_{-11,12},\vec{s})=1$. Also, notice that for every $\beta'_{11}<\beta^*_{ii}$ it must be the case that $x_1(\beta'_{11}, 0_{12}, \vec{\beta}_{-11,12},\vec{s})=0$. This follow from monotonicity and the fact that  $x_1(\beta'_{11}, \vec{\beta}_{-11},\vec{s})=0$ for every $\beta'_{11}<\beta^*_{ii}$. Therefore, although agent 1 gets the item both when she declares $v_1 = c s_1 + s_2/c$ and  $v_1 = c s_1$, her utility is 
$$\beta^*_{11}+1/c - p_1(0_{11}, 1/c, \vec{\beta}_{-11,12}, \vec{s})$$ 
when she reports the former, while paying 
$$\beta^*_{11} - p_1(0_{11}, 0_{12}, \vec{\beta}_{-11,12}, \vec{s})$$ 
when she reports the latter. For ex-post IC mechanisms, it must imply 
\begin{align} \label{eqn:imp_eq1}
	1/c - p_1(0_{11}, 1/c, \vec{\beta}_{-11,12}, \vec{s}) = - p_1(0_{11}, 0_{12}, \vec{\beta}_{-11,12}, \vec{s}).
\end{align}
By our construction, if the mechanism achieves a better than $c$ approximation, $x_1(0_{11}, 1/c, \vec{\beta}_{-11,12}, \vec{s})=0$ and $x_1(0_{11}, 0_{12}, \vec{\beta}_{-11,12}, \vec{s})=0$, which means that agent $1$ will not get the item when she reports $v_1 = s_2/c$ or $v_1 = 0$. But her payments for the two reports are different according to~\eqref{eqn:imp_eq1}, which is contradictory to ex-post IC.

